Learning Transformer-based World Models with Contrastive Predictive Coding

The DreamerV3 algorithm recently obtained remarkable performance across diverse environment domains by learning an accurate world model based on Recurrent Neural Networks (RNNs). Following the success of model-based reinforcement learning algorithms and the rapid adoption of the Transformer architecture for its superior training efficiency and favorable scaling properties, recent works such as STORM have proposed replacing RNN-based world models with Transformer-based world models using masked self-attention. However, despite the improved training efficiency of these methods, their impact on performance remains limited compared to the Dreamer algorithm, struggling to learn competitive Transformer-based world models. In this work, we show that the next state prediction objective adopted in previous approaches is insufficient to fully exploit the representation capabilities of Transformers. We propose to extend world model predictions to longer time horizons by introducing TWISTER (Transformer-based World model wIth contraSTivE Representations), a world model using action-conditioned Contrastive Predictive Coding to learn high-level temporal feature representations and improve the agent performance. TWISTER achieves a human-normalized mean score of 162% on the Atari 100k benchmark, setting a new record among state-of-the-art methods that do not employ look-ahead search.

==> tables/atari100k+dreamer_pro.tex <==
\begin{table}[ht]
    \caption{Agent scores and human-normalized metrics on the 26 games of the Atari 100k benchmark. We show average scores over 5 seeds. Bold numbers indicate best performing method for each game.}
    \centering
    \setlength{\tabcolsep}{3pt}
    \scriptsize
    \hfill \break
    \begin{tabular}{lrrrrrrrrrr}
    \toprule
    Game & Random & Human & SimPLe & DreamerPro & TWM & IRIS & DreamerV3 & STORM & $\Delta$-IRIS & TWISTER (ours) \\ 
    \midrule
    Alien & 228 & 7128  & 617 & 635 & 675 & 420 & 959 & \textbf{984} & 391 & 970 \\
    Amidar & 6 & 1720  & 74 & 85 & 122 & 143 & 139 & \textbf{205} & 64 & 184 \\
    Assault & 222 & 742  & 527 & 374 & 683 & \textbf{1524} & 706 & 801 & 1123 & 721 \\
    Asterix & 210 & 8503  & 1128 & 594 & 1116 & 854 & 932 & 1028 & \textbf{2492} & 1306 \\
    Bank Heist & 14 & 753 & 34 & 217 & 467 & 53 & 649 & 641 & \textbf{1148} & 942 \\
    Battle Zone & 2360 & 37188 & 4031 & 4200 & 5068 & 13074 & 12250 & \textbf{13540} & 11825 & 9920 \\
    Boxing & 0 & 12 & 8 & 84 & 78 & 70 & 78 & 80 & 70 & \textbf{88} \\
    Breakout & 2 & 30 & 16 & 14 & 20 & 84 & 31 & 16 & \textbf{302} & 35\\
    Chopper Command & 811 & 7388 & 979 & 1564 & 1697 & 1565 & 420 & \textbf{1888} & 1183 & 910 \\
    Crazy Climber & 10780 & 35829 & 62584 & 53964 & 71820 & 59324 & \textbf{97190} &  66776 & 57854 & 81880 \\
    Demon Attack & 152 & 1971 & 208 & 123 & 350 & \textbf{2034} & 303 & 165 & 533 & 289 \\
    Freeway & 0 & 30 & 17 & 11 & 24 & 31 & 0 &  \textbf{34} & 31 & 32 \\
    Frostbite & 65 & 4335 & 237 & 723 & \textbf{1476} & 259 & 909 & 1316 & 279 & 305  \\
    Gopher & 258 & 2412 & 597 & 1250 & 1675 & 2236 & 3730 & 8240 & 6445 & \textbf{22234} \\
    Hero & 1027 & 30826 & 2657 & 4331 & 7254 & 7037 & \textbf{11161} & 11044 & 7049 & 8773 \\
    James Bond & 29 & 303 & 100 & 142 & 362 & 463 & 445 & 509 & 309 & \textbf{573} \\
    Kangaroo & 52 & 3035 & 51 & 2040 & 1240 & 838 & 4098 & 4208 & 2269 & \textbf{6016} \\
    Krull & 1598 & 2666 & 2205 & 6989 & 6349 & 6616 & 7782 & 8413 & 5978 & \textbf{8839} \\
    Kung Fu Master & 258 & 22736 & 14862 & 20650 & 24555 & 21760 & 21420 & \textbf{26182} & 21534 & 23442 \\
    Ms Pacman & 307 & 6952 & 1480 & 1240 & 1588 & 999 & 1327 & \textbf{2673}  & 1067 & 2206 \\
    Pong & –21 & 15 & 13 & 3 & 19 & 15 & 18 & 11 & \textbf{20} & \textbf{20} \\
    Private Eye & 25 & 69571 & 35 & 40 & 87 & 100 & 882 & \textbf{7781} & 103 & 1608\\ 
    Qbert & 164 & 13455 & 1289 & 1094 & 3331 & 746 & 3405 & \textbf{4522} & 1444 & 3197\\
    Road Runner & 12 & 7845 & 5641 & 9122 & 9107 & 9615 & 15565 & 17564 & 10414 & \textbf{17832} \\ 
    Seaquest & 68 & 42055 & 683 & 366 & \textbf{774} & 661 & 618 & 525 & 827 & 532 \\
    Up N Down & 533 & 11693 & 3350 & 4021 & \textbf{15982} & 3546 & 7600 & 7985 & 4072 & 7068\\
    \midrule
    \# Superhuman & 0 & N/A & 1 & 4 & 8 & 10 & 9 & 10 & 11 & \textbf{12} \\
    Normed Mean (\%) & 0 & 100 & 33 & 79 & 96 & 105 & 112 & 127 & 139 & \textbf{\resultmean}\\
    Normed Median (\%) & 0 & 100 & 13 & 28 & 51 & 29 & 49 & 58 & 53 & \textbf{\resultmedian} \\
    \bottomrule
    \end{tabular}
    \label{table:results_atari100k}
\end{table}
